Sample-Efficient Learning of Correlated Equilibria in Extensive-Form Games

Imperfect-Information Extensive-Form Games (IIEFGs) is a prevalent model for real-world games involving imperfect information and sequential plays. The Extensive-Form Correlated Equilibrium (EFCE) has been proposed as a natural solution concept for multi-player general-sum IIEFGs. However, existing algorithms for finding an EFCE require full feedback from the game, and it remains open how to efficiently learn the EFCE in the more challenging bandit feedback setting where the game can only be learned by observations from repeated playing. This paper presents the first sample-efficient algorithm for learning the EFCE from bandit feedback. We begin by proposing $K$-EFCE -- a more generalized definition that allows players to observe and deviate from the recommended actions for $K$ times. The $K$-EFCE includes the EFCE as a special case at $K=1$, and is an increasingly stricter notion of equilibrium as $K$ increases. We then design an uncoupled no-regret algorithm that finds an $\varepsilon$-approximate $K$-EFCE within $\widetilde{\mathcal{O}}(\max_{i}X_iA_i^{K}/\varepsilon^2)$ iterations in the full feedback setting, where $X_i$ and $A_i$ are the number of information sets and actions for the $i$-th player. Our algorithm works by minimizing a wide-range regret at each information set that takes into account all possible recommendation histories. Finally, we design a sample-based variant of our algorithm that learns an $\varepsilon$-approximate $K$-EFCE within $\widetilde{\mathcal{O}}(\max_{i}X_iA_i^{K+1}/\varepsilon^2)$ episodes of play in the bandit feedback setting. When specialized to $K=1$, this gives the first sample-efficient algorithm for learning EFCE from bandit feedback.

==> new_version/new_algorithm.tex <==

% For any sequence of policies $\{\pi^t\}_{t=1}^T$, we also define the \emph{counterfactual loss function} (for the $t$-th round) $\{L_{i,h}^t(x_{i,h}, a_{i,h})\}_{i,h,x_{i,h},a_{i,h}}$ as~\citep{zinkevich2007regret}: 
% % \sm{$\cA_{-i}$ not defined}
% {\small
% \begin{align}
%     & \l_{i,h}^t(x_{i,h}, a_{i,h}) \defeq \sum_{\substack{s_h\in x_{i,h}, \\ \ba_{-i,h}\in\mc{A}_{-i}}} p_{1:h}(s_h) \prod_{j\neq i} \pi_{j, 1:h}^t(x_{j}(s_h), a_{j,h}) [1 - r_{i,h}(s_h, \ba_h)], \label{equation:l-definition} \\
%     & \L_{i,h}^{t}(x_{i,h}, a_{i,h}) \defeq \l_{i,h}^t(x_{i,h}, a_{i,h}) + \sum_{h'=h+1}^H \sum_{\substack{x_{h'}\in \cC_{h'}(x_{i, h}, a_{i,h}), \\ a_{h'}\in\mc{A}_i}} \pi_{i,(h+1):h'}^t(x_{h'}, a_{h'}) \l_{i,h'}^t(x_{h'}, a_{h'}). \label{equation:L-definition}
% \end{align}
% }Intuitively, $\L_{i,h}^{t}(x_{i,h}, a_{i,h})$ measures the \ith player's expected loss (one minus reward) conditioned on reaching $(x_{i,h}, a_{i,h})$, weighted by the (environment) transitions and all other players' policies $\pi_{-i}^t$ at all time steps, and the \ith player's own policy $\pi_i^t$ from step $h+1$ onward. We will omit the $i$ subscript and use $L_h^t$ to denote the above when clear from the context.



\def\Regalg{{\textsc{RegAlg}}}

\begin{algorithm}[t]
  \small
   \caption{\kefr~ with full feedback~(\ith player's version)}
   \label{algorithm:kefr-fullfeedback}
   \begin{algorithmic}[1]
     \REQUIRE Algorithm for regret minimization with time selection and strategy modification \Regalg. 
     \STATE Initialize regret minimizers $\{\regmin_{x_{i,h}}\}_{x_{i,h}\in\cX_i}$ with $\Regalg$. \ziang{$\cB^s$ and $\cB^e$}
     \FOR{iteration $t=1,\dots,T$}
     \FOR{$h=1,\dots,H$} 
     \FOR{$x_{i,h}\in\mc{X}_{i,h}$}
     \STATE Compute $S^t_{b_{1:h-1}} = \prod_{k = 1}^{h-1} \pi_{i, k}^t(b_k \vert x_k)$ for $b_{1: h - 1} \in \omegai(x_{i, h})$. \label{line:Sb-for-typeI} 
     \STATE Compute $S^t_{b_{1:h_\star}} = \prod_{k = 1}^{h_\star} \pi_{i, k}^t(b_k \vert x_k)$ for $b_{1: h_\star} \in \omegaii(x_{i, h})$.  \label{line:Sb-for-typeII} 
     \STATE $\regmin_{x_{i,h}}.\observe( \{ S^t_{b_{1:h - 1}} \}_{b_{1:h - 1} \in \omegai(x_{i, h})} \cup \{ S^t_{b_{1:h_\star}} \}_{b_{1:h_\star} \in \omegaii(x_{i, h})})$.
     \STATE Set policy $\pi_i^t(x_{i, h}) \setto \regmin_{x_{i,h}} .\recommend()$.  
     \ENDFOR
     \ENDFOR
     \STATE\label{line:observe-loss}  Compute counterfactual losses $\set{L_h^t(x_{i,h}, a_h)}_{h, x_{i,h}, a_h}$ (depending on $\pi_i^t$ and $\pi_{-i}^t$; cf.~\eqref{equation:L-definition}) 
     \FOR{all $x_{i,h}\in\cX_i$}\label{line:begin-update}
     \STATE $\regmin_{x_{i,h}}.\observe( \set{ L_h^t(x_{i,h}, a)}_{a\in\cA_i} )$. \label{line:regmin-s}
     \ENDFOR
     \ENDFOR
     \ENSURE Policies $\{ \pi_i^t \}_{t \in [T]}$. 
 \end{algorithmic}
\end{algorithm}
